Causal Interventions for Fairness

Most approaches in algorithmic fairness constrain machine learning methods so the resulting predictions satisfy one of several intuitive notions of fairness. While this may help private companies comply with non-discrimination laws or avoid negative publicity, we believe it is often too little, too late. By the time the training data is collected, individuals in disadvantaged groups have already suffered from discrimination and lost opportunities due to factors out of their control. In the present work we focus instead on interventions such as a new public policy, and in particular, how to maximize their positive effects while improving the fairness of the overall system. We use causal methods to model the effects of interventions, allowing for potential interference--each individual's outcome may depend on who else receives the intervention. We demonstrate this with an example of allocating a budget of teaching resources using a dataset of schools in New York City.

==> depricated.tex <==
% old section 2
\section{Method}
Imagine we have a set of $n$ individuals. Each individual $i$ has a set of features $\Xc_i$, where $\Xc_i$ is a set of $d$ random variables. Also each individual belongs to a sensitive group $A_i$ (similarly $A_i$ is a random variable). For each individual $i$ we may decide to perform an intervention $Z_i$ (for simplicity we will assume throughout that $A_i, Z_i$ are binary). Finally, after a possible intervention, each individual has some outcome $Y_i$.

In general, each outcome $Y_i$ is influenced by an individual's sensitive group $A_i$, features $\Xc_i$, and the intervention $Z_i$
\begin{align}
A_i \rightarrow Y_i \;\;\;\;\;\; \Xc_i \rightarrow Y_i \;\;\;\;\;\; Z_i \rightarrow Y_i \nonumber
\end{align}
where $\rightarrow$ signifies a \emph{direct} causal influence via a structural equation model (SEM) as described by \cite{pearl:00,pearl:16}. At the same time, we believe that the neighbors of $i$, defined as $N(i)$, influence $i$. Specifically, their interventions will influence the outcome of $i$: $\{Z_j\}_{j \in N(i)} \xdashrightarrow{} Y_i$, where $\xdashrightarrow{}$ signifies either an \emph{indirect} or direct `spillover' causal effect. Figure~\ref{fig:example} shows a simple example where two individuals are neighbors and thus, there are (possibly) indirect `spillover' effects from their individual interventions.
\begin{wrapfigure}{R}{0.5\textwidth}
\begin{center}
%\vspace{-14ex}
\centerline{\includegraphics[width=0.5\textwidth]{fig/simple_itt.pdf}}
%\vspace{-2ex}
  \caption{\small An example causal diagram with interventions $Z$, outcomes $Y$, features $\Xc$, and sensitive group $A$. Here, individuals $1,3$ are neighbors of individual $2$, thus their interventions may `spillover' in possibly indirect ways, as shown by the dashed arrows.\label{fig:example}}
\end{center}
\vspace{-10ex}
\end{wrapfigure}

\paragraph{Objective.}
Without considering fairness, our goal is to assign beneficial interventions $Z$ to maximize the sum of expected outcomes over individuals with a maximum budget $B$ (we assume we are always implicitly conditioning on features $\Xc$, thus we omit $\Xc$ in all equations for clarity):
\begin{align}
\max_{Z_1, \ldots, Z_n} \sum_{i=1}^n&\; \mathbb{E}_{p(Y_i | Z_i, A_i)}[Y_i]  \nonumber \\
s.t., \;\sum_{i=1}^n&\; Z_i \leq B \nonumber
\end{align}
However, even though such an intervention may be applied without considering an individual's sensitive group $A$, being a member of a certain group may cause individuals to have different outcomes.

\paragraph{Example 1: Job recruitment.}
For instance, consider that $Z$ is a job-training program for information technology (IT) jobs. This is a free program that boosts ones chances of obtaining an IT job (i.e., outcome $Y\!=\!1$). Let $\Xc$ be relevant features such as one's school grades and interview performance. Let the sensitive group $A$ be gender. Now imagine, in Figure~\ref{fig:example}, individual $1$ is female and individual $2$ is male.
As a female, individual $1$, was pressured by her peers and teachers throughout her schooling to study for `more suitable' fields. This made it harder to study and despite her high work ethic and natural aptitude for IT, caused her school grades to be worse than they would have been had she not had to deal with this pressure. 
On the other hand, individual $2$, a male, was encouraged by his friends and teachers to study IT. Despite, this he decided to not spend very much effort and so achieved average grades.
Because, the program only had enough funds to fund one more person, and individual $1$ had slightly worse grades (due to prejudice), individual $2$ was selected to undergo the job-training program ($Z\!=\!1$).
Afterwards, they both applied for the same job and both got interviews. Individual $1$ spoke less and appeared less confident than individual $2$, who wore a suit and talked comfortably about things he had learned in the training program. Thus, individual $2$ got the job.

\paragraph{Example 2: College admissions.}
TODO
\paragraph{Example 3: Directing police officers.}
TODO

\subsection{Reducing Societal Privilege}
In the above cases, interventions were given to individuals because they had benefited previously from their group-privilege: the man was thought to be more suited for IT, which resulted in slightly better grades, despite the fact that the woman worked harder. In this section we describe how to measure an individual's group-privilege, we then use this measure to learn to allocate interventions to those who benefit the least from privilege.

\paragraph{Measuring group-privilege.}
The key observation is that if someone is group-privileged then their outcome $Y_i$ should be very different from their outcome had they been in a different sensitive group $A$. This hypothetical outcome can be quantified by a counterfactual: $Y_i(a')$ is the outcome individual $i$ would have had if they had been a member of a different group $a'$. Assuming we can compute this counterfactual (which we describe in detail in the following section), then we can measure group-privilege as follows:
   \begin{align}
\underbrace{\mathbb{E}_{p(Y_i | Z_i, A_i)}[Y_i] - \mathbb{E}_{p(Y_i(a') | Z_i, A_i)}[Y_i(a')]}_{G_i} \nonumber
\end{align}
This quantity measures the increase in someone's outcome due to their group under any intervention, assuming binary groups (this could be easily extended to multiple groups by averaging). If it is positive then being in their group has benefited them, and if negative, being in their group has harmed them. The magnitude tells us the strength of this effect.

\paragraph{Learning interventions.}
To learn interventions that reduce group-privilege we propose to incorporate the above measure as a constraint:
\begin{align}
\max_{Z_1, \ldots, Z_n} \sum_{i=1}^n&\; \mathbb{E}_{p(Y_i | Z_i, A_i)}[Y_i]  \label{eq:opt} \\
s.t., \;\sum_{i=1}^n&\; Z_i \leq B \nonumber \\
&\; G_i \leq \tau \;\;\; \forall i \in 1,\ldots,n. \nonumber
\end{align}
Where $\tau \geq 0$ indicates the amount of allowed positive group privilege. As $\tau$ varies we obtain a solution path similar to other shrinkage operators such as the LASSO (CITE).


\paragraph{Alternative formulations.}
Instead of the difference between two expectations we could also formulate the constraint as $P(Y_i - Y_i(a') \leq \tau \mid Z_i, A_i)$.

% Thus, to avoid these interventions having or emphasizing discriminatory effects, we propose to measure the discrimination of an intervention as follows:
% \begin{align}
% \overbrace{\Big| \mathbb{E}_{p(Y_{i}^{A_i \leftarrow 0} | Z_i = 0, A_i)}[Y_i] - \mathbb{E}_{p(Y_{i}^{A_i \leftarrow 1} | Z_i = 0, A_i)}[Y_i] \Big|}^{D_0^i} \nonumber \\
% \overbrace{\Big| \mathbb{E}_{p(Y_{i}^{A_i \leftarrow 0} | Z_i = 1, A_i)}[Y_i] - \mathbb{E}_{p(Y_{i}^{A_i \leftarrow 1} | Z_i = 1, A_i)}[Y_i] \Big|}^{D_1^i} \nonumber
% \end{align}
% where $Y_{i}^{A_i \leftarrow 0}$ is the counterfactual random variable where an individual's sensitive attribute $A_i$ is set to value $0$. $D^i_0$ is the absolute discrimination to individual $i$ \emph{without an intervention} (i.e., $Z\!=\!0$), and $D^i_1$ is the absolute discrimination \emph{with intervention}. 

% To ensure interventions are not discriminatory we propose to learn interventions that maximize the total expected outcomes while \emph{not increasing discrimination}:
% \begin{align}
% \max_{Z_1, \ldots, Z_n}& \sum_{i=1}^n \mathbb{E}_{p(Y_i | Z_i, A_i)}[Y_i] \nonumber \\
% s.t.,& \; D_1^i \leq D_0^i, \;\; \forall i \nonumber 
% \end{align}

% Note that, to evaluate each $G_i$ we must be able to compute the marginal counterfactual distribution $Y_i(a')$ for $a' \neq A_i$ for each individual. If instead we wished to compute the probability $P(Y_i - Y_i(a') \leq tau)$ then we need to be able to compute the difference between two unknown random variables.

% then we would need the joint counterfactual distribution over four counterfactuals: $Y_i^{A_i \leftarrow 0}|Z_i=0,Y_i^{A_i \leftarrow 1}|Z_i=0,Y_i^{A_i \leftarrow 0}|Z_i=1,Y_i^{A_i \leftarrow 1}|Z_i=1$. 


% we wished to compute the expectation outside of the absolute value we would need to be able to compute the joint counterfactual distribution $Y_i^{A_i \leftarrow 0},Y_i^{A_i \leftarrow 1}$. If instead we wished to compute the probability $P(D_1^i \leq D_0^i)$ then we would need the joint counterfactual distribution over four counterfactuals: $Y_i^{A_i \leftarrow 0}|Z_i=0,Y_i^{A_i \leftarrow 1}|Z_i=0,Y_i^{A_i \leftarrow 0}|Z_i=1,Y_i^{A_i \leftarrow 1}|Z_i=1$. 

\subsection{Optimization}
As mentioned, we assume $Z_1, \ldots, Z_n$ are a set of binary random variables. There are many possible ways to solve for this, which use different assumptions:

Thus, to solve for the above optimization problem, the we propose to model the above expectations as:
\begin{align}
\mathbb{E}_{p(Y_i | Z_i = z_i, A_i = a_i)}[Y_i] = a_i (w_1^i z_i + w_0^i (1-z_i)) \mathbf{x}_i  \sum_{j \in N(i)} (w_1^{ij} z_j + w_0^{ij} (1 - z_j)) \nonumber 
\end{align}
where $w_0^i,w_1^i,w_0^{ij},w_1^{ij}$ are weights that change depending on the value of interventions on individuals $i$ and $j$, and are fixed quantities.
As we have modeled this expectation as a linear function of $Z_i$ the optimization problem in eq.~\ref{eq:opt} is an integer linear program (ILP). Two ideas for solving this are:
\begin{enumerate}
\item Relax the program to a linear program (by allowing Z to be real-valued), then solve using the simplex algorithm and round the solution to the nearest integer values.
\item Somehow form the problem as a constrained submodular optimization problem via lagrange multipliers.
\end{enumerate}
